Combining Self-labeling with Selective Sampling

Since data is the fuel that drives machine learning models, and access to labeled data is generally expensive, semi-supervised methods are constantly popular. They enable the acquisition of large datasets without the need for too many expert labels. This work combines self-labeling techniques with active learning in a selective sampling scenario. We propose a new method that builds an ensemble classifier. Based on an evaluation of the inconsistency of the decisions of the individual base classifiers for a given observation, a decision is made on whether to request a new label or use the self-labeling. In preliminary studies, we show that naive application of self-labeling can harm performance by introducing bias towards selected classes and consequently lead to skewed class distribution. Hence, we also propose mechanisms to reduce this phenomenon. Experimental evaluation shows that the proposed method matches current selective sampling methods or achieves better results.

==> figures/schema.tex <==
\begin{tikzpicture}[
squarednode/.style={rectangle, draw, minimum size=5mm},
]
%Nodes
\node [] (input) {x};

\node [] (anchor) [right=0.8cm of input] {};

\node [] (anchor_model2) [above=0.1cm of anchor] {};
\node [] (anchor_model1) [above=0.5cm of anchor_model2] {};
\node [] (anchor_dots) [below=0.0cm of anchor] {};
\node [] (anchor_model3) [below=0.5cm of anchor_dots] {};

\node [squarednode, minimum width=15mm] (model2) [right=0.3cm of anchor_model2] {$f_2$};
\node [squarednode, minimum width=15mm] (model1) [right=0.3cm of anchor_model1] {$f_1$};
\node [minimum width=15mm] (dots) [right=0.3cm of anchor_dots] {$\vdots$};
\node [squarednode, minimum width=15mm] (model3) [right=0.3cm of anchor_model3] {$f_L$};

\node [squarednode, minimum width=7mm] (prediction1) [right=0.8cm of model1] {$\hat{y}_1$};
\node [squarednode, minimum width=7mm] (prediction2) [right=0.8cm of model2] {$\hat{y}_2$};
\node [minimum width=7mm] (dots_pred) [right=0.8cm of dots] {$\vdots$};
\node [squarednode, minimum width=7mm] (prediction3) [right=0.8cm of model3] {$\hat{y}_L$};

\node[] (anchor_out) [right=3.9cm of anchor] {};
\node [] (anchor_out_model2) [right=0.6cm of prediction2] {}; %[above=0.5cm of anchor_out] {};
\node [] (anchor_out_model1) [right=0.6cm of prediction1] {}; %[above=0.5cm of anchor_out_model2] {};
\node [] (anchor_out_model3) [right=0.6cm of prediction3] {}; %[below=0.5cm of anchor_out] {};

\node [squarednode, align=center] (check) [right=0.3cm of anchor_out] {confidence and\\consistency check};

\node [] (anchor_if) [right=0.5cm of check] {};
\node [] (failed) [above=0.8cm of anchor_if] {FAILED};
\node [] (anchor_if_up) [above=0.8cm of failed] {};
\node [] (passed) [below=0.8cm of anchor_if] {PASSED};
\node [] (anchor_if_down) [below=0.8cm of passed] {};

\node [squarednode, align=center, minimum width=17mm] (oracle) [right=0.5cm of anchor_if_up] {request\\label};
\node [] (anchor_AL) [right=0.3cm of oracle] {};
\node [squarednode, align=center] (training1) [right=0.2 of anchor_AL] {bootstrapped\\training};
\node [squarednode, align=center, minimum width=17mm] (filter) [right=0.5cm of anchor_if_down] {prior\\filter};
\node [] (anchor_SL) [right=0.3cm of filter] {};
\node [squarednode, align=center] (training2) [right=0.2 of anchor_SL] {bootstrapped\\training};

\node[align=center] (input_description) [above=0.2cm of input] {Unlabeled\\data};
\node[] (ensemble) [above=0.2cm of model1] {ensemble};
\node[] (predictions) [right=0.3cm of ensemble] {predictions};
\node[align=center] (AL) [above=0.3cm of anchor_AL] {Training with label from annotator\\(Active Learning)};
\node[align=center] (SL) [below=0.4cm of anchor_SL] {Training with predicted label\\(Self-labeling)};

%Lines
\draw[-] (input.east) -- (anchor.center);
\draw[-] (anchor.center) -- (anchor_model1.center);
\draw[-] (anchor.center) -- (anchor_model3.center);

\draw[->] (anchor_model1.center) -- (model1);
\draw[->] (anchor_model2.center) -- (model2);
\draw[->] (anchor_model3.center) -- (model3);

\draw[->] (model1) -- (prediction1);
\draw[->] (model2) -- (prediction2);
\draw[->] (model3) -- (prediction3);

\draw[-] (prediction1) -- (anchor_out_model1.center);
\draw[-] (prediction2) -- (anchor_out_model2.center);
\draw[-] (prediction3) -- (anchor_out_model3.center);
\draw[-] (anchor_out_model1.center) -- (anchor_out.center);
\draw[-] (anchor_out_model3.center) -- (anchor_out.center);
\draw[->] (anchor_out.center) -- (check);

\draw[-] (check.east) -- (anchor_if.center);
\draw[-] (anchor_if.center) -- (failed.south);
\draw[-] (failed.north) -- (anchor_if_up.center);
\draw[-] (anchor_if.center) -- (passed.north);
\draw[-] (passed.south) -- (anchor_if_down.center);

\draw[->] (anchor_if_up.center) -- (oracle.west);
\draw[->] (oracle) -- (training1);
\draw[->] (anchor_if_down.center) -- (filter.west);
\draw[->] (filter) -- (training2);

\end{tikzpicture}

==> tables/batch.tex <==
\begin{tabular}{c|c|c|c|c|c|c|c|c|c}
    \multirow{2}{*}{dataset} & \multirow{2}{*}{method} & \multicolumn{2}{c}{batch 100} & \multicolumn{2}{c}{batch 200} & \multicolumn{2}{c}{batch 500} & \multicolumn{2}{c}{full training} \\
    \cline{3-10} 
     & & accuracy & training time & accuracy & training time & accuracy & training time & accuracy & training time \\
     \hline 
     wine & random & 0.4226 & 0m9,538s & 0.4207 & 0m9,525s & 0.4055 & 0m9,469s
     & 0.4429 & 0m15,417s \\
     & fixed uncertainty & 0.3948 & 0m9,749s & 0.4132 & 0m9,904s & 0.4132 & 0m9,782s & 0.4058 & 0m10,808s \\
     & variable uncertainty & 0.3863 & 0m9,772s & 0.3977 & 0m9,691s & 0.3682 & 0m9,747s & 0.4162 & 0m15,981s \\
     & classification margin & 0.4505 & 0m9,968s & 0.4111 & 0m9,775s & 0.4234 & 0m9,888s & 0.4150 & 0m12,623s \\
    & vote entropy & 0.4070 & 0m43,519s & 0.4179 & 0m42,956s & 0.4268 & 0m43,572s & 0.4466 & 1m37,661s \\
    & SL2S & 0.4170 & 0m45,803s & 0.4164 & 0m45,687s & 0.4344 & 0m44,597s & 0.4419 & 2m9,664s \\
    \hline
    abalone & random & 0.1688 & 0m10,647s & 0.1805 & 0m10,544s & 0.1783 & 0m10,459s & 0.1852 & 0m14,888s \\
     & fixed uncertainty & 0.1977 & 0m10,497s & 0.1816 & 0m10,568s & 0.2012 & 0m10,582s & 0.1921 & 0m15,023s \\
     & variable uncertainty & 0.1709 & 0m10,615s & 0.1892 & 0m10,605s & 0.1946 & 0m10,660s & 0.1851 & 0m15,111s \\
     & classification margin & 0.1982 & 0m10,679s & 0.1831 & 0m10,591s & 0.1887 & 0m10,580 & 0.1909 & 0m14,924s \\
     & vote entropy & 0.2125 & 0m56,880s & 0.1975 & 0m55,759s & 0.1992 & 0m56,268s & 0.1869 & 1m37,354s \\
     & SL2S & 0.2137 & 0m58,620s & 0.2204 & 0m57,749s & 0.1787 & 0m58,300s & 0.2105 & 1m57,304s \\
     \hline
    nursery & random & 0.9877 & 0m45,721s & 0.9650 & 0m45,929s & 0.9530 & 0m46,539s & 0.9998 & 1m24,814s \\
    & fixed uncertainty & 0.9234 & 0m46,527s & 0.8914 & 0m46,235s & 0.8914 & 0m46,117s & 0.9617 & 0m46,993s \\
    & variable uncertainty & 0.9960 & 0m46,261s & 0.9962 & 0m44,500s & 0.9747 & 0m46,252s & 1.0 & 1m33,338s \\
    & classification margin & 0.9522 & 0m46,188s & 0.9403 & 0m46,485s & 0.8914 & 0m46,707s & 0.9899 & 0m47,453s \\
    & vote entropy & 0.9747 & 3m2,867s & 0.9688 & 3m16,535s & 0.9407 & 3m7,318s & 0.9998 & 11m13,531s \\
    & SL2S & 0.9742 & 3m37,875s & 0.9678 & 3m33,953s & 0.9558 & 3m35,028s & 1.0 & 5m4,965s \\
    \hline
    firewall & random & 0.9977 & 11m32,076s & 0.9930 & 11m21,547s & 0.9899 & 11m21,097s & 0.9962 & 50m24,495s \\
    & fixed uncertainty & 0.9877 & 11m24,445s & 0.9898 & 11m25,752s & 0.9898 & 11m28,198s & 0.9910 & 11m24,864s \\
    & variable uncertainty & 0.9963 & 11m34,387s & 0.9955 & 11m28,516s & 0.9916 & 11m25,953s & 0.9979 & 49m37,772s \\
    & classification margin & 0.9906 & 11m23,074s & 0.9900 & 11m20,269s & 0.9897 & 11m29,806s & 0.9923 & 11m17,467s \\
    & vote entropy & 0.9963 & 72m23,903s & 0.9977 & 73m26,329s & 0.9918 & 77m28,704s & 0.9980 & 435m18,893s \\
    & SL2S & 0.9895 & 76m54,044s & 0.9899 & 74m38,641s & 0.9897 & 78m25,423s & - & - \\
    \hline
\end{tabular}

==> tables/big.tex <==
\begin{tabular}{l|ccccc}
\hline 
& \multicolumn{5}{c}{dataset adult} \\ 
\hline 
 all labeled           &  & & 0.741±0.010 & & \\
 all labeled ensemble   & & &  0.756±0.005  & & \\
\hline 
budget & 0.1 & 0.2 & 0.3 & 0.4 & 0.5 \\ 
\hline 
 random                 &  0.735±0.007  &  0.733±0.005  &  0.729±0.007  &  0.731±0.005  &  0.732±0.006 \\
 fixed uncertainty      &  0.754±0.007  &  0.758±0.008  &  0.765±0.009  &  0.760±0.011  &  0.760±0.011 \\
 variable uncertainty   &  0.756±0.013  &  0.751±0.011  &  0.755±0.012  &  0.758±0.012  &  0.746±0.011 \\
 classification margin  &  0.757±0.008  &  0.757±0.008  &  0.757±0.008  &  0.757±0.008  &  0.757±0.008 \\
 consensus entropy      &  0.764±0.004  & \textbf{  0.767±0.005  } &  0.765±0.002  &  0.765±0.004  &  0.764±0.003 \\
 min margin             & \textbf{  0.768±0.004  } & \textbf{  0.767±0.005  } & \textbf{  0.768±0.004  } & \textbf{  0.768±0.004  } & \textbf{  0.768±0.004 } \\
 SL2S                   &  0.762±0.003  &  0.763±0.004  &  0.763±0.004  &  0.762±0.003  &  0.762±0.004 \\
 
\hline 
& \multicolumn{5}{c}{dataset bank marketing} \\ 
\hline 
 all labeled & & & 0.712±0.012 & & \\
 all labeled ensemble   & & & 0.714±0.009 & & \\
\hline
budget & 0.1 & 0.2 & 0.3 & 0.4 & 0.5 \\ 
\hline 
 random                 &  0.700±0.023  &  0.694±0.017  &  0.703±0.021  &  0.698±0.014  &  0.699±0.018 \\
 fixed uncertainty      &  0.691±0.014  &  0.710±0.014  &  0.705±0.019  &  0.705±0.019  &  0.705±0.019 \\
 variable uncertainty   &  0.690±0.014  &  0.694±0.018  &  0.700±0.018  &  0.703±0.013  &  0.697±0.018 \\
 classification margin  &  0.682±0.012  &  0.682±0.012  &  0.682±0.012  &  0.682±0.012  &  0.682±0.012 \\
 consensus entropy      &  0.701±0.011  &  0.714±0.007  & \textbf{  0.719±0.006  } &  0.715±0.009  &  0.715±0.009 \\
 min margin             &  0.705±0.006  & \textbf{  0.716±0.007  } &  0.716±0.007  &  0.716±0.007  &  0.716±0.007 \\
 SL2S                   & \textbf{  0.709±0.007  } &  0.715±0.009  &  0.718±0.009  & \textbf{  0.719±0.008  } & \textbf{  0.718±0.009 } \\

\hline
& \multicolumn{5}{c}{dataset firewall} \\ 
\hline 
 all labeled           & & & 0.997±0.001 & & \\
 all labeled ensemble  & & & 0.998±0.000 & &  \\
\hline 
budget & 0.1 & 0.2 & 0.3 & 0.4 & 0.5 \\ 
\hline 
 random                 &  0.996±0.002  & \textbf{  0.997±0.002  } & \textbf{  0.998±0.001  } & \textbf{  0.997±0.001  } & \textbf{  0.998±0.001 } \\
 fixed uncertainty      &  0.993±0.002  &  0.996±0.002  &  0.996±0.002  &  0.996±0.002  &  0.996±0.002 \\
 variable uncertainty   &  0.994±0.002  & \textbf{  0.997±0.001  } &  0.997±0.001  & \textbf{  0.997±0.001  } &  0.997±0.001 \\
 classification margin  &  0.991±0.001  &  0.991±0.001  &  0.991±0.001  &  0.991±0.001  &  0.991±0.001 \\
 consensus entropy      &  0.992±0.001  &  0.992±0.001  &  0.992±0.001  &  0.992±0.001  &  0.992±0.001 \\
 min margin             &  0.991±0.001  &  0.991±0.001  &  0.991±0.001  &  0.991±0.001  &  0.991±0.001 \\
 SL2S                   & \textbf{  0.997±0.001  } & \textbf{  0.997±0.001  } &  0.997±0.001  & \textbf{  0.997±0.001  } &  0.997±0.001 \\


\hline 
& \multicolumn{5}{c}{dataset chess} \\ 
\hline 
 all labeled           &       &       & 0.816±0.011 &       &       \\
 all labeled ensemble   &         &         &  0.850±0.007  &         &        \\
\hline 
budget & 0.1 & 0.2 & 0.3 & 0.4 & 0.5 \\ 
\hline 
 random                 & \textbf{  0.515±0.017  } &  0.581±0.015  &  0.630±0.009  &  0.669±0.014  &  0.698±0.009 \\
 fixed uncertainty      &  0.459±0.017  &  0.538±0.015  &  0.593±0.017  &  0.639±0.017  &  0.674±0.014 \\
 variable uncertainty   &  0.464±0.021  &  0.543±0.016  &  0.604±0.016  &  0.651±0.016  &  0.691±0.014 \\
 classification margin  &  0.466±0.019  &  0.543±0.015  &  0.606±0.013  &  0.653±0.014  &  0.692±0.014 \\
 consensus entropy      &  0.492±0.016  & \textbf{  0.594±0.009  } & \textbf{  0.662±0.008  } & \textbf{  0.715±0.010  } & \textbf{  0.758±0.009 } \\
 min margin             &  0.491±0.022  &  0.589±0.017  &  0.660±0.016  &  0.713±0.016  &  0.752±0.014 \\
 SL2S                   &  0.491±0.013  &  0.585±0.010  &  0.655±0.012  &  0.702±0.010  &  0.748±0.010 \\

 \hline
\end{tabular}

==> tables/data_loading_big.tex <==
\begin{tabular}{c|c|c|c}
    \hline
    dataset & \pbox{1.5cm}{numeric features} & \pbox{2cm}{categorical features} & target feature \\
    \hline
    nursery &
    - & 
    \pbox{2cm}{parents, has nurs, form, children,\\ housing, finance, social} &
    CLASS
    \\
    \hline
    mushroom &
    - & 
    \pbox{1.5cm}{cap-shape, cap-color} &
    class
    \\
    \hline
    wine & 
    \pbox{2cm}{fixed acidity, volatile acidity, \\ citric acid, residual sugar, \\ chlorides, free sulfur dioxide,\\ total sulfur dioxide, density, pH,\\ sulphates, alcohol} & 
    - &
    quality 
    \\
    \hline
    abalone & 
    \pbox{2cm}{Length, Diameter, Height, \\ Whole weight, Shucked weight,\\ Viscera weight, Shell weight} & 
    Sex &
    Rings 
    \\
    \hline
\end{tabular}
